Nonparametric estimation of the purity of a quantum state in quantum homodyne tomography with noisy data

The aim of this work is to estimate a quadratic functional of a unknown Wigner function from noisy tomographic data. The Wigner function can be seen as the representation of the quantum state of a light beam. The estimation of a quadratic functional is done from result of quantum homodyne measurement performed on identically prepared quantum systems. We start by constructing an estimator of a quadratic functional of the Wigner function. We show that the proposed estimator is optimal or nearly optimal in a minimax sense over a class of infinitely differentiable functions. Parametric rates are also reached for some values of the smoothness parameters and the asymptotic normality is given. Then, we construct an adaptive estimator that does not depend on the smoothness parameters and prove it is minimax over some set-ups.

==> bibkatia.tex <==
@article {BickelRitov,
    AUTHOR = {Bickel, P. J. and Ritov, Y.},
     TITLE = {Estimating integrated squared density derivatives: sharp best
              order of convergence estimates},
   JOURNAL = {Sankhy\=a (Statistics). The Indian Journal of Statistics.
              Series A},
  FJOURNAL = {Sankhy\=a (Statistics). The Indian Journal of Statistics.
              Series A},
    VOLUME = {50},
      YEAR = {1988},
    NUMBER = {3},
     PAGES = {381--393},
      ISSN = {0581-572X},
     CODEN = {SANABS},
   MRCLASS = {62G05 (62G20)},
  MRNUMBER = {MR1065550 (91e:62079)},
}
@article {MR1331653,
    AUTHOR = {Birg\'{e}, Lucien and Massart, Pascal},
     TITLE = {Estimation of integral functionals of a density},
   JOURNAL = {The Annals of Statistics},
  FJOURNAL = {The Annals of Statistics},
    VOLUME = {23},
      YEAR = {1995},
    NUMBER = {1},
     PAGES = {11--29},
      ISSN = {0090-5364},
     CODEN = {ASTSC7},
   MRCLASS = {62G05},
  MRNUMBER = {MR1331653 (96c:62065)},
MRREVIEWER = {Margaret P. Gessaman},
}
@article {MR1394973,
    AUTHOR = {Kerkyacharian, G\'{e}rard and Picard, Dominique},
     TITLE = {Estimating nonquadratic functionals of a density using {H}aar
              wavelets},
   JOURNAL = {The Annals of Statistics},
  FJOURNAL = {The Annals of Statistics},
    VOLUME = {24},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {485--507},
      ISSN = {0090-5364},
     CODEN = {ASTSC7},
   MRCLASS = {62G05 (62G20)},
  MRNUMBER = {MR1394973 (97e:62062)},
MRREVIEWER = {Michael Falk},
}
@article {MR1394981,
    AUTHOR = {Laurent, B\'{e}atrice},
     TITLE = {Efficient estimation of integral functionals of a density},
   JOURNAL = {The Annals of Statistics},
  FJOURNAL = {The Annals of Statistics},
    VOLUME = {24},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {659--681},
      ISSN = {0090-5364},
     CODEN = {ASTSC7},
   MRCLASS = {62G05 (62G20)},
  MRNUMBER = {MR1394981 (97d:62079)},
MRREVIEWER = {Philippe Vieu},
}
@Article{MR1772223,
author = {Tribouley, K.},
title = {Adaptive estimation of integrated functionals},
journal = {Mathematical Methods of Statistics},
year = {2000},
OPTkey = {},
OPTvolume = {9},
OPTnumber = {1},
OPTpages = {19--38},
OPTmonth = {},
OPTnote = {},
OPTannote = {}
}
@Article{GoldSpok06,
author = {Goldenshluger, A. and Spokoiny, V.},
title = {Recovering convex edges of an image from noisy tomographic data},
journal = {IEEE Transactions on Information Theory},
year = {2006},
OPTkey = {},
OPTvolume = {52},
OPTnumber = {4},
OPTpages = {1322--1334},
OPTmonth = {April},
OPTnote = {},
OPTannote = {}
}
@article {MR1790012,
    AUTHOR = {Cavalier, Laurent},
     TITLE = {Efficient estimation of a density in a problem of tomography},
   JOURNAL = {The Annals of Statistics},
  FJOURNAL = {The Annals of Statistics},
    VOLUME = {28},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {630--647},
      ISSN = {0090-5364},
     CODEN = {ASTSC7},
   MRCLASS = {62G07},
  MRNUMBER = {MR1790012 (2001h:62060)},
MRREVIEWER = {B. L. S. Prakasa Rao},
}
@article {MR1041393,
    AUTHOR = {Johnstone, Iain M. and Silverman, Bernard W.},
     TITLE = {Speed of estimation in positron emission tomography and
              related inverse problems},
   JOURNAL = {The Annals of Statistics},
  FJOURNAL = {The Annals of Statistics},
    VOLUME = {18},
      YEAR = {1990},
    NUMBER = {1},
     PAGES = {251--280},
      ISSN = {0090-5364},
     CODEN = {ASTSC7},
   MRCLASS = {62G05 (62C20 62P10 65U05)},
  MRNUMBER = {MR1041393 (91c:62038)},
MRREVIEWER = {T. Robertson},
}
@Book{Leon97,
author = {Ulf Leonhardt},
ALTeditor = {},
title = {Measuring the Quantum State of Light},
publisher = {Cambridge University Press},
year = {1997},
OPTkey = {},
OPTvolume = {},
OPTnumber = {},
OPTseries = {},
OPTaddress = {},
OPTedition = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {}
}
@Article{Vogelrisken,
  title = {Determination of quasiprobabiltity distributions in terms of 
probability distributions for rotated quadrature phase},
  author = {Vogel, K. and Risken, H.},
  journal = {Physical Review},
  volume = {A},
  number = {40},
  pages = {2847--2849},
  numpages = {},
  year = {1989},
  month = {March},
  doi = {},
  publisher = {}
}
@Article{SmitA,
  title = {Measurement of the Wigner distribution and the density matrix of a light mode using optical homodyne tomography: Application to squeezed states and the vacuum},
  author = {Smithey, D. T. and Beck, M.  and Raymer, M. G. and Faridani, A.},
  journal = {Physical Review Letters},
  volume = {70},
  number = {9},
  pages = {1244--1247},
  numpages = {3},
  year = {1993},
  month = {March},
  doi = {10.1103/PhysRevLett.70.1244},
  publisher = {American Physical Society}
}
@Article{Smitheybis,
  title = {Experimental determination of number-phase uncertainty relations},
  author = {Smithey, D.J. and Beck, M. and Cooper, M.J. and  Raymer, M. G.},
  journal = {Optics Letters},
  volume = {18},
  number = {},
  pages = {1259--1261},
  numpages = {},
  year = {1993},
  month = {},
  doi = {},
  publisher = {}
}
@Unpublished{GutaArt05,
author = {Madalin Gu{\c{t}}{\u{a}} and Luis Artiles},
title = {Minimax estimation of the Wigner in quantum homodyne tomography with ideal detectors},
note = {Manuscrit},
OPTkey = {},
OPTmonth = {},
OPTyear = {2006},
OPTannote = {}
}
@book {MR1226450,
    AUTHOR = {Korostel{\"e}v, A. P. and Tsybakov, A. B.},
     TITLE = {Minimax theory of image reconstruction},
    SERIES = {Lecture Notes in Statistics},
    VOLUME = {82},
PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1993},
     PAGES = {xii+258},
      ISBN = {0-387-94028-6},
   MRCLASS = {62G05 (62G20 62H11 62M30 68U10)},
  MRNUMBER = {MR1226450 (95a:62028)},
MRREVIEWER = {Mauro Piccioni},
}
@article {ButGutArt05,
    AUTHOR = {Cristina Butucea and Madalin Gu{\c{t}}{\u{a}} and Luis Artiles},
     TITLE = {Minimax and adaptive estimation of the Wigner function in quantum homodyne tomography with noisy data},
   JOURNAL = {The Annals of Statistics},
  FJOURNAL = {},
    VOLUME = {to appear},
      YEAR = {2006},
    NUMBER = {},
     PAGES = {},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
}
@article {MR2136642,
    AUTHOR = {Artiles, L. M. and Gill, R. D. and Gu{\c{t}}{\u{a}}, M. I.},
     TITLE = {An invitation to quantum tomography},
   JOURNAL = {Journal of the Royal Statistical Society. Series B. Statistical Methodology},
  FJOURNAL = {Journal of the Royal Statistical Society. Series B. Statistical Methodology},
    VOLUME = {67},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {109--134},
      ISSN = {1369-7412},
   MRCLASS = {81P15 (62G05 62G07 81V80)},
  MRNUMBER = {MR2136642 (2006d:81016)},
}
@Article{GoldZeev06,
author = {Alexander Goldenshluger and Assaf Zeevi},
title = {Recovering convex boundaries from blurred and noisy observations},
journal = {The Annals of Statistics},
year = {2006},
OPTkey = {},
OPTvolume = {34},
OPTnumber = {3},
OPTpages = {1375-1394},
OPTmonth = {},
OPTnote = {},
OPTannote = {}
}
@article{GoldSpok04,
    AUTHOR = {Goldenshluger, A. and Spokoiny, V.},
     TITLE = {On the shape-from-moments problem and recovering edges from noisy {R}adon data},
   JOURNAL = {Probability Theory and Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {128},
      YEAR = {2004},
    NUMBER = {1},
     PAGES = {123--140},
      ISSN = {0178-8051},
     CODEN = {PTRFEU},
   MRCLASS = {44A12 (44A60 62C20 62G20 62H12 62H35 94A08 94A12)},
  MRNUMBER = {MR2027297 (2004k:44001)},
MRREVIEWER = {Fritz Keinert},
}
@TechReport{Butu04,
author = {Cristina Butucea},
title = {Quadratic functional estimation in view of minimax goodness-of-fit testing from noisy data},
institution = {No.936, Universit\'{e} Paris VI},
year = {2004},
OPTkey = {},
OPTtype = {936},
OPTnumber = {},
OPTaddress = {},
OPTmonth = {},
OPTnote = {},
OPTannote = {}
}
@article{ButuTsyba04,
    AUTHOR = {Cristina Butucea and Alexandre Tsybakov},
     TITLE = {Sharp optimality for density deconvolution with dominating bias},
   JOURNAL = {Theory of Probability and its Applications},
  FJOURNAL = {},
    VOLUME = {to appear},
      YEAR = {2006},
    NUMBER = {},
     PAGES = {},
      ISSN = {},
     CODEN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
}

